Multi-Document Grounded Multi-Turn Synthetic Dialog Generation

We introduce a technique for multi-document grounded multi-turn synthetic dialog generation that incorporates three main ideas. First, we control the overall dialog flow using taxonomy-driven user queries that are generated with Chain-of-Thought (CoT) prompting. Second, we support the generation of multi-document grounded dialogs by mimicking real-world use of retrievers to update the grounding documents after every user-turn in the dialog. Third, we apply LLM-as-a-Judge to filter out queries with incorrect answers. Human evaluation of the synthetic dialog data suggests that the data is diverse, coherent, and includes mostly correct answers. Both human and automatic evaluations of answerable queries indicate that models fine-tuned on synthetic dialogs consistently out-perform those fine-tuned on existing human generated training data across four publicly available multi-turn document grounded benchmark test sets.

==> answerability_correctness_correlation.tex <==
\begin{table}
\small
\centering
\begin{tabular}{cccc}\\\hline
\textbf{Turn Depth}  & \textbf{\#Turns} & \textbf{\%correct} & \textbf{\%answerable}  \\\hline
1 & 100 & 76.8 & 87.5 \\
2  & 120  & 68.2 & 83.7 \\
3  & 180  & 66.4 & 79.3  \\
4  & 232  & 77.9 & 87.8 \\
5  & 80  & 84.4 & 93.8  \\\hline
Overall  & 712 & 73.1 & 85.2  \\\hline
\end{tabular}
\caption{Correlation between query answerability and response correctness. Out of the 220 annotations with unanswerable queries, 193 (87.7\%) had incorrect responses. Out of the 1270 annotations with answerable queries, 1062 (83.6\%) had correct answers, as opposed to the overall 73.1 \%correct.}
\label{tab:correlation-between-answerability-correctness}
\end{table}

==> benchmark_baseline_table.tex <==
\begin{table*}[h]
\centering
\small
\begin{tabular}{llcccc}\hline
\textbf{Models} & \textbf{TestSet} & \textbf{F1} & \textbf{RougeL} & \textbf{Bert-Recall} & \textbf{Recall} \\\hline
LlaMa2-13B-Chat & or-quac & 0.149 & 0.144  & 0.196  & 0.290   \\
 & multidoc2dial & 0.250  & 0.220 & 0.282  & 0.363   \\
             & quac    & 0.295 & 0.306  & 0.319   & 0.447    \\\hline
Merlinite-7B  & or-quac & 0.164  & 0.162  &  0.200 & 0.278 \\
 & multidoc2dial & 0.279 & 0.251 & 0.339 & 0.456 \\
             & quac & 0.364  & 0.377 & 0.347  & 0.478 \\\hline

\end{tabular}
\caption{Zero-shot baseline experimental results on the three benchmark evaluation data sets with the base models merlinite-7b, llama2-13b-chat}
\label{tab:benchmark_zeroshot_baseline_evaluation}
\end{table*}
% Note: zero-shot baseline w/ model-runner vs. tst scores for bert-k-prec & k-prec scores are vastly different ... Since I am using tst inferencing for the rest of the experiments, I will be switching to tst scores for the zero shot later for consistency 
% Will be tracking down the cause for the very difference (bert-)k-prec scores later

\begin{comment}
\begin{table*}[h]
\centering
\small
\begin{tabular}{l|l|cccccc}\hline
 & & \textbf{F1} & \textbf{RougeL} & \textbf{Bert-Recall} & \textbf{Recall} & \textbf{Bert-KPrec} & \textbf{K-Precision} \\\hline
             & OR-QuAC-syn & 0.156  & 0.155  &  0.190  & 0.267  & 0.165 & 0.741 \\
             & OR-QuAC-gold & 0.273 & 0.266  & 0.336 & 0.481 & 0.313 & 0.829 \\
Merlinite-7B & MD2D &  &   &   &    &    &  \\
             & QuAC & 0.322  & 0.333 & 0.302  & 0.443 & 0.209 & 0.796 \\\hline
             & OR-QuAC-syn & 0.146   & 0.142 & 0.198 & 0.287  & 0.167  &  0.709 \\
             & OR-QuAC-gold & 0.243 & 0.235 & 0.326 & 0.456 & 0.371 & 0.798 \\
LlaMa2-13B-Chat & MD2D &   &  &   &   &  &  \\
             & QuAC    & 0.270  & 0.282  & 0.276   & 0.403   & 0.380 & 0.840 \\\hline


\end{tabular}
\caption{Zero-shot baseline experimental results on the three benchmark development data sets with the base models merlinite-7b, llama2-13b-chat}
\label{tab:benchmark_zeroshot_baseline_evaluation}
\end{table*}
\end{comment}
% llama2-13b-chat: LlaMa_wrapper
% merlinite-7b: ModelFactoryGraniteLabWrapper

==> benchmark_data_comparison_table.tex <==
\begin{table}
\centering
%\small
\begin{tabular}{l|c|c|c|c|c}
\hline
\textbf{Dataset} & \textbf{OR} & \textbf{IS} & \textbf{DG} & \textbf{MD} & \textbf{RAG} \\
\hline
CoQA & H & N  & Y & N & N \\
%QuAC & H & Y & Y & N  & N \\
OR-QuAC & H & Y & Y & N & Y \\
MD2D & H & Y & Y & Y & N \\
Beize & N & N & N & N & N \\
Dynamic-RAG & N & Y & Y & Y & Y \\\hline
\end{tabular}
\caption{Comparison of Multi-turn Benchmark Dataset for origin (OR), human (H) or synthetic (S), information seeking (IS), document grounded (DG), multiple document (MD), retrieval-augmented (RAG). MD2D denotes MultiDoc2Dial and Dynamic-RAG, our work.}
\label{tab:benchmark_data_comparison}
\end{table}

==> benchmark_sft.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{llcccc}\hline
\textbf{Benchmarks/Models} & \textbf{TrainSet} & \textbf{F1} & \textbf{RougeL} & \textbf{Bert-Recall} & \textbf{Recall} \\\hline
\textbf{CoQA} \\\hline
 & zero-shot & 0.234 & 0.226   & 0.218 & 0.406 \\
LlaMA-13B-Chat & benchmark  & 0.376 &	0.377 &	0.089 &	0.318 \\
 & synthetic & 0.426 &	0.426 &	0.223 &	0.425 \\
 & benchmark \& synthetic & 0.397  &	0.400  &	0.193  &	0.371 \\\hline
 & zero-shot  & 0.261 &  0.254 &  0.241 & 0.444  \\
 Merlinite-7B & benchmark  &  0.379 &	0.382 &	0.092 &	0.321  \\
  & synthetic & 0.441 & 	0.438 & 	0.306 & 0.495  \\
  & benchmark \& synthetic & 0.410 &	0.402 &	0.162 &	0.361\\\hline
\textbf{MultiDoc2Dial} \\\hline
 & zero-shot & 0.250 & 0.220 & 0.282 & 0.363 \\
LlaMA-13B-Chat & benchmark & 0.547 & 0.531 & 0.534 & 0.543 \\
 & synthetic & 0.432 & 0.312 & 0.412 & 0.361 \\
 & benchmark \& synthetic & 0.560 & \textbf{0.549} & \textbf{0.563} & \textbf{0.570} \\\hline
 & zero-shot & 0.279 & 0.251 & 0.339 & 0.456 \\
 Merlinite-7B & benchmark & 0.547 & 0.531 & 0.534 & 0.543 \\
  & synthetic & 0.424 & 0.302 & 0.402 & 0.355\\
  & benchmark \& synthetic & \textbf{0.566} & 0.542 & 0.551 & 0.554 \\\hline
\textbf{QuAC}  (1000)          \\\hline
Mixtral-8X7B-Instruct & zero-shot & 0.243 & 0.250 & 0.305 & 0.500 \\\hline
  & zero-shot & 0.284 & 0.295 & 0.292 & 0.448 \\
LlaMA-13B-Chat & benchmark & 0.525 & 0.538 & 0.468 & 0.531 \\
 & synthetic & 0.438 & 0.447 & 0.415 & 0.499 \\
 & benchmark \& synthetic & 0.536 & 0.547 & 0.483 & 0.545 \\\hline
  & zero-shot & 0.234 & 0.241 & 0.263 & 0.444 \\
Merlinite-7B & benchmark & 0.538 & 0.550 & 0.472 & 0.539 \\
 & synthetic & 0.418 & 0.427 & 0.410 & 0.499 \\
 & benchmark \& synthetic & \textbf{0.546} & \textbf{0.558} & \textbf{0.491} & \textbf{0.550} \\\hline
\textbf{OR-QuAC} (5571) \\\hline
Mixtral-8X7B-Instruct & zero-shot & 0.155 & 0.148 & 0.209 &  0.301 \\\hline
     & zero-shot  & 0.099 & 0.095 & 0.109 & 0.201 \\
LlaMA-13B-Chat & benchmark & 0.281 & 0.284 & 0.203 & 0.289 \\
 & synthetic & 0.219 & 0.219 & 0.228 & 0.248 \\
 & benchmark \& synthetic & 0.281  & 0.284 & 0.268 & 0.286 \\
\hline
   & zero-shot  & 0.138 & 0.137 & 0.152 & 0.214 \\
Merlinite-7B & benchmark & 0.285 & 0.288 & 0.277 & 0.290 \\
            & synthetic & 0.202  & 0.201  & 0.229 & 0.255  \\
            & benchmark \& synthetic & 0.292 & 0.294 & 0.285 & 0.298 \\\hline
\end{tabular}
\caption{Benchmark testset performances on models fined-tuned on various types of training data}
\label{tab:benchmark_sft_evaluation}
\end{table*}

\begin{comment}
\begin{table*}[h]
\small
\centering
\begin{tabular}{lllcccc}\hline
\textbf{Benchmarks/Models} & \textbf{TrainSet} & \textbf{TestSet} & \textbf{F1} & \textbf{RougeL} & \textbf{Bert-Recall} & \textbf{Recall} \\\hline
\textbf{CoQA} \\\hline
 & zero-shot & CoQA &  &  &  &  \\
LlaMA-13B-Chat & CoQA & CoQA & 0.376 &	0.377 &	0.089 &	0.318 \\
 & mr-CoQA & CoQA & 0.426 &	0.426 &	0.223 &	0.425 \\
 & mr-CoQA\&CoQA & CoQA & 0.397  &	0.400  &	0.193  &	0.371 \\\hline
 & zero-shot & CoQA &  &  &  &  \\
 Merlinite-7B & CoQA & CoQA &  0.379 &	0.382 &	0.092 &	0.321  \\
  & mr-CoQA & CoQA & 0.441 & 	0.438 & 	0.306 & 0.495  \\
  & mr-CoQA\&CoQA & CoQA & 0.410 &	0.402 &	0.162 &	0.361\\\hline
\textbf{MultiDoc2Dial} \\\hline
 & zero-shot & md2d & 0.250 & 0.220 & 0.282 & 0.363 \\
LlaMA-13B-Chat & md2d & md2d & 0.547 & 0.531 & 0.534 & 0.543 \\
 & mr-md2d & md2d & 0.432 & 0.312 & 0.412 & 0.361 \\
 & mr-md2d\&md2d & md2d & 0.560 & \textbf{0.549} & \textbf{0.563} & \textbf{0.570} \\\hline
 & zero-shot & md2d & 0.279 & 0.251 & 0.339 & 0.456 \\
 Merlinite-7B & md2d & md2d & 0.547 & 0.531 & 0.534 & 0.543 \\
  & mr-md2d & md2d & 0.424 & 0.302 & 0.402 & 0.355\\
  & mr-md2d\&md2d & md2d & \textbf{0.566} & 0.542 & 0.551 & 0.554 \\\hline
\textbf{QuAC}  (1000)          \\\hline
  & zero-shot & quac & 0.295 & 0.306 & 0.319 & 0.447 \\
LlaMA-13B-Chat & quac & quac & 0.525 & 0.538 & 0.468 & 0.531 \\
% & mr-quac-st & quac & 0.357 & 0.389 & 0.252 & 0.364 \\
 & mr-quac & quac & 0.438 & 0.447 & 0.415 & 0.499 \\
 & mr-quac\&quac & quac & 0.536 & 0.547 & 0.483 & 0.545 \\\hline
  & zero-shot & quac & 0.364 & 0.377 & 0.347 & 0.478 \\
Merlinite-7B & quac & quac & 0.538 & 0.550 & 0.472 & 0.539 \\
% & mr-quac-st & quac & 0.380 & 0.389 & 0.394 & 0.526 \\
 & mr-quac & quac & 0.418 & 0.427 & 0.410 & 0.499 \\
 & mr-quac\&quac & quac & \textbf{0.546} & \textbf{0.558} & \textbf{0.491} & \textbf{0.550} \\\hline
\textbf{OR-QuAC} (5571) \\\hline
     & zero-shot & or-quac & 0.149 & 0.144 & 0.196 & 0.290 \\
LlaMA-13B-Chat &or-quac & or-quac & 0.281 & 0.284 & 0.203 & 0.289 \\
 % & dr-quac-st & or-quac & 0.184 & 0.182 & 0.170 & 0.196 \\
 & dr-quac & or-quac & 0.219 & 0.219 & 0.228 & 0.248 \\
 & dr-\&or-quac & or-quac & 0.281  & 0.284 & 0.268 & 0.286 \\
 \cline{2-7}
& mr-quac & or-quac-dr & 0.283 & 0.282 & 0.294 & 0.333 \\
& dr-quac & or-quac-dr & 0.302 & 0.300 & 0.314 & 0.360 \\
& dr-\&or-quac & or-quac-dr & 0.419 & 0.421 & 0.393 & 0.426 \\\hline
   & zero-shot & or-quac & 0.154 & 0.152 & 0.181 & 0.256 \\
Merlinite-7B & or-quac & or-quac & 0.285 & 0.288 & 0.277 & 0.290 \\
%& dr-quac-st & or-quac &  &  &  & \\
            & dr-quac & or-quac & 0.202  & 0.201  & 0.229 & 0.255  \\
            & dr-\&or-quac & or-quac & 0.292 & 0.294 & 0.285 & 0.298 \\
            \cline{2-7}
             & mr-quac & or-quac-dr & 0.272 & 0.268  & 0.308 & 0.372 \\
             & dr-quac & or-quac-dr & 0.282  & 0.278  & 0.313 & 0.374 \\
             & dr-\&or-quac & or-quac-dr & 0.428  & 0.430 & 0.412 & 0.441
             \\\hline


\end{tabular}
\caption{Benchmark data performance of models fined-tuned on various types of training data}
\label{tab:benchmark_sft_evaluation}
\end{table*}
\end{comment}

==> coqa_table.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{lllcccc}\hline
\textbf{Benchmarks/Models} & \textbf{QueryType} & \textbf{TrainSet} & \textbf{F1} & \textbf{RougeL} & \textbf{Bert-Recall} & \textbf{Recall} \\\hline
\textbf{CoQA scored with Rationale as reference}            \\\hline
LlaMA-13B-Chat & answerable & original  & 0.378 &	0.379 &	0.088 &	0.320	 \\
 & (7918)  & synthetic  & \textbf{0.430} &	\textbf{0.430} &	\textbf{0.226} &	\textbf{0.428}   \\
        \cline{2-7}
 & unanswerable & original   & 0.139 &	0.139 &	0.159 &	0.139	  \\
 &  (65)   & synthetic    & 0.015 &	0.015 &	0.109 &	0.015  \\
\hline
Merlinite-7B & answerable & original  &  0.381 &	0.384 &	0.092 &	0.323  \\
 & (7918)  &  synthetic  &  \textbf{0.445} &	\textbf{0.441} &	\textbf{0.311} &	\textbf{0.499}  \\
        \cline{2-7}
 & unanswerable & original &  0.108 &	0.108 &	0.113 &	0.108  \\
 &  (65)   & synthetic &  0.015 &	0.015 &	0.099 &	0.015 \\
\hline
\textbf{CoQA scored with Short Answer as reference} \\\hline
LlaMA-13B-Chat & answerable & original  & \textbf{0.811} & \textbf{0.807} &	\textbf{0.734} &	0.813	 \\
 & (7918)  & synthetic  & 0.667 &	0.663 &	0.629 &	\textbf{0.834}   \\
        \cline{2-7}
 & unanswerable & original  & 0.151	& 0.151 &	0.171 &	0.152	  \\
 &  (65)   & synthetic    & 0.015 &	0.015 &	 0.11 &	0.015  \\
\hline
Merlinite-7B & answerable & original  &  \textbf{0.819} & \textbf{0.816} & \textbf{0.741} &	0.821  \\
 & (7918)  &  synthetic  &  0.532 &	0.528 &	0.525 &	\textbf{0.854}  \\
        \cline{2-7}
 & unanswerable & original &  0.106 &	0.106 &	0.118	& 0.106  \\
 &  (65)   & synthetic &  0.015 &	0.015 &	0.13 &	0.016 \\
\hline
\end{tabular}
\caption{CoQA automatic scores according to two types of references: One with reference answer (short) and the other with rationale (long).}
\label{tab:coqa-answer-vs-rationale}
\end{table*}

==> interannotatoragreement.tex <==
\begin{table}
\centering
\begin{tabular}{llll}\\\hline
           &  \textbf{E} & \textbf{H} & \textbf{R} \\\hline
\textbf{C} & 90 (45/50) & 65 (71/110) & 77 (46/60) \\
\textbf{E} &         & 74 (37/50) & 72 (43/60) \\
\textbf{H} &         &       & 42 (50/120) \\\hline
\end{tabular}
\caption{Inter-annotator agreement (IAA) w.r.t the response correctness across 4 annotators, C, E, H and R. Included in parentheses are raw numbers. Agreement rate ranges from the lowest 42\% to the highest 90\%.}
\label{tab:IAA}
\end{table}

==> mrc-algorithm.tex <==
\begin{algorithm}[t]
\small
\caption{Single-document Grounded Dialog Generation}
\label{alg:mrc-dialog-algorithm}
\textbf{Input}: Grounding document $doc_{g}$ \\
\textbf{Output}: $dialog_{n}$ 

\begin{algorithmic}[1]
\STATE $history \leftarrow \phi$  

%\FOR{ i = 1}
%\STATE $q_{1} \leftarrow LLM(doc_{g})$
%\STATE $r_{1} \leftarrow LLM(q_{1}, doc_{g})$ \\
%\STATE $history_{1} \leftarrow q_{1}~\cup~r_{1}$ \\
%\ENDFOR

\FOR {$i$ in $1~...~n$}
\STATE $q_{i} \leftarrow LLM(history_{i-1}, doc_{g}$)
\STATE $r_{i} \leftarrow LLM(q_{i}, history_{i-1}, doc_{g}$)
\STATE $history_{i} \leftarrow 
 history_{i-1} \cup q_{i} \cup r_{i}$

\ENDFOR
\STATE $dialog_{n} \leftarrow history_{n}$
\STATE return $dialog_{n}$
\end{algorithmic}
\end{algorithm}



==> only_answerable_test_table.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{llcccc}\hline
\textbf{Benchmarks/Models} & \textbf{TrainSet} & \textbf{F1} & \textbf{RougeL} & \textbf{Bert-Recall} & \textbf{Recall} \\\hline
\textbf{QuAC} (665)           \\\hline
Mixtral-8X7B-Instruct-v0.1 & zero-shot & 0.295 & 0.292  & 0.382  & \textbf{\textbf{0.525}} \\\hline
               & zero-shot & 0.325  & 0.324 & 0.393 & \textbf{0.513} \\
LlaMA2-13B-Chat & benchmark  & 0.366 & 0.379 & 0.299 & 0.373 \\
 &   synthetic  & \textbf{0.393} & \textbf{0.395} & \textbf{0.402} & 0.479  \\\hline
        & zero-shot & 0.294 & 0.290 & 0.374 & 0.509 \\
Merlinite-7B & benchmark & 0.367 & 0.382 & 0.282 & 0.368 \\
   &  synthetic & \textbf{0.399} & \textbf{0.396} & \textbf{0.442} & \textbf{0.531} \\
\hline
\textbf{OR-QuAC} (4421)          \\\hline
Mixtral-8X7B-Instruct-v0.1 & zero-shot & 0.191  & 0.183   &  \textbf{0.256} & \textbf{0.367}  \\\hline
                & zero-shot  & 0.122 & 0.118   &  0.132   &  0.244     \\
LlaMA2-13B-Chat & benchmark  & 0.145 & 0.149 & 0.133 & 0.153 \\
 & synthetic  & 0.153 & 0.154 & 0.163 & 0.187 \\
\hline
             & zero-shot & 0.168  & 0.166 & 0.186  & 0.262  \\
Merlinite-7B & benchmark & 0.142  & 0.145 & 0.130  & 0.149 \\
  & synthetic & \textbf{0.199} & \textbf{0.197} & 0.233 & 0.265 \\
\hline
\textbf{MD2D} (6178)           \\\hline
Mixtral-8X7B-Instruct-v0.1 & zero-shot &  &   &    &  \\\hline
                & zero-shot &    &      &      &     \\
LlaMA2-13B-Chat & benchmark  & 0.406 &	0.389 &	0.376 &	0.407 \\
   &  synthetic  & \textbf{0.429} &	\textbf{0.407} & \textbf{0.412} &	\textbf{0.493} \\
\hline
              & zero-shot  &  &  &  &  \\
Merlinite-7B  & benchmark  & 0.409 & 0.392 & 0.394 &	0.430  \\
   & synthetic  & \textbf{0.439} & \textbf{0.421} & \textbf{0.415} & \textbf{0.450} \\
\hline
\textbf{CoQA} w/ rationale (7918)           \\\hline
Mixtral-8X7B-Instruct-v0.1 & zero-shot &   &   &    &     \\\hline
               & zero-shot &      &     &      &    \\
LlaMA2-13B-Chat & benchmark  & 0.378 &	0.379 &	0.088 &	0.320	 \\
 & synthetic  & \textbf{0.430} &	\textbf{0.430} &	\textbf{0.226} &	\textbf{0.428}   \\
\hline
            & zero-shot &      &       &          &     \\
Merlinite-7B & benchmark  &  0.381 &	0.384 &	0.092 &	0.323  \\
  &  synthetic  &  \textbf{0.445} &	\textbf{0.441} &	\textbf{0.311} &	\textbf{0.499}  \\
\hline
\textbf{CoQA} w/ short answer (7918) \\\hline
Mixtral-8X7B-Instruct-v0.1 & zero-shot &    &     &      &    \\\hline
                & zero-shot &    &      &      &   \\
LlaMA2-13B-Chat & benchmark  & \textbf{0.811} & \textbf{0.807} &	\textbf{0.734} &	0.813	 \\
  & synthetic  & 0.667 &	0.663 &	0.629 &	\textbf{0.834}   \\
\hline
            & zero-shot &       &      &       &      \\
Merlinite-7B  & benchmark  &  \textbf{0.819} & \textbf{0.816} & \textbf{0.741} &	0.821  \\
  &  synthetic  &  0.532 &	0.528 &	0.525 &	\textbf{0.854}  \\
\hline
\end{tabular}
\caption{Benchmark testset performances on \textbf{answerable queries}. Comparison is between models fine-tuned on \textit{human annotated benchmark} training data vs. \textit{synthetic} data . Models fine-tuned only on synthetic data only consistently out-perform those fine-tuned on the benchmark data. The only exception is the CoQA data set scored with short answer as reference for which the models trained on synthetic data perform better than those on the benchmark data for Recall only. However, we show in \S{\ref{sec:human-evaluation}} that humans overwhelmingly prefer outputs generaed by the models fine-tuned only synthetic data to those by the models trained on the benchmark data.}
\label{tab:only-answerable-results}
\end{table*}

\begin{comment}
\begin{table*}[h]
\small
\centering
\begin{tabular}{lllcccc}\hline
\textbf{Benchmarks/Models} & \textbf{QueryType} & \textbf{TrainSet} & \textbf{F1} & \textbf{RougeL} & \textbf{Bert-Recall} & \textbf{Recall} \\\hline
\textbf{QuAC}            \\\hline
LlaMA-13B-Chat & answerable & benchmark  & 0.366 & 0.379 & 0.299 & 0.373 \\
 & (665)  &  synthetic  & \textbf{0.393} & \textbf{0.395} & \textbf{0.402} & \textbf{0.479}  \\
        \cline{2-7}
 & unanswerable & benchmark & 0.843   & 0.852  & 0.805  & 0.844  \\
 &  (335)            & synthetic & 0.527  & 0.550  & 0.440  & 0.540 \\\hline
Merlinite-7B & answerable & benchmark & 0.367 & 0.382 & 0.282 & 0.368 \\
   & (665) & synthetic & \textbf{0.394} & \textbf{0.393} & \textbf{0.431} & \textbf{0.509} \\
          \cline{2-7}
    & unanswerable & benchmark & 0.879 & 0.888 & 0.852 & 0.881 \\
    & (335) & synthetic & 0.467 & 0.494 & 0.366 & 0.479 \\
\hline
\textbf{OR-QuAC}            \\\hline
LlaMA-13B-Chat & answerable & benchmark  & 0.145 & 0.149 & 0.133 & 0.153 \\
 & (4421)  & synthetic  & \textbf{0.153} & \textbf{0.154}  & \textbf{0.163} & \textbf{0.187} \\
        \cline{2-7}
 & unanswerable & benchmark & 0.799   & 0.799  & 0.799  & 0.799  \\
 &  (1150)  & synthetic & 0.468  &  0.465  & 0.469  & 0.472 \\
\hline
Merlinite-7B & answerable & benchmark & 0.142  & 0.145 & 0.130  & 0.149 \\
   & (4421) & synthetic & \textbf{0.199} & \textbf{0.197} & \textbf{0.233} & \textbf{0.265} \\
          \cline{2-7}
    & unanswerable & benchmark & 0.841  & 0.841 & 0.841 & 0.841  \\
    & (1150) & synthetic & 0.215  & 0.215 & 0.216 & 0.217  \\
\hline

\textbf{MD2D}            \\\hline
LlaMA-13B-Chat & answerable & benchmark  & 0.406 &	0.389 &	0.376 &	0.407 \\
 & (6178)  &  synthetic  & \textbf{0.429} &	\textbf{0.407} & \textbf{0.412} &	\textbf{0.493} \\
        \cline{2-7}
 & unanswerable & benchmark &  0.766 &	0.753 &	0.779 &	0.755  \\
 &  (4026)   & synthetic &  0.461 & 0.441 &	0.580 &	0.611 \\
\hline
Merlinite-7B & answerable & benchmark  & 0.409 & 0.392 & 0.394 &	0.430  \\
 & (6178)  &  synthetic  & \textbf{0.439} & \textbf{0.421} & \textbf{0.415} & \textbf{0.450} \\
        \cline{2-7}
 & unanswerable & benchmark &  0.769 &	0.756 &	0.787 &	0.765  \\
 &  (4026)   & synthetic &  0.410 &	0.403 &	0.546 &	0.585  \\
\hline

\end{tabular}
\caption{Benchmark testset performance according to answerable vs. unanswerable query types. Comparison is between models fine-tuned on human annotated benchmark training data only vs. synthetic data only. For answerable queries, models fine-tuned only on synthetic data consistently out-perform those fine-tuned on human annotated data or combination of the two (not shown in the table due to its similarity in scores to models fine-tuned on human generated data only except that scores on answerable queries are slightly higher and unanswerable queries, slightly lower).}
\label{tab:answerable-vs-unanswerable-results}
\end{table*}
\end{comment}

\begin{comment}
\begin{table*}[h]
\small
\centering
\begin{tabular}{lllcccc}\hline
\textbf{Benchmarks/Models} & \textbf{QueryType} & \textbf{TrainSet} & \textbf{F1} & \textbf{RougeL} & \textbf{Bert-Recall} & \textbf{Recall} \\\hline
\textbf{QuAC}            \\\hline
LlaMA-13B-Chat & answerable & quac  & 0.366 & 0.379 & 0.299 & 0.373 \\
 & (665)  &  mr-quac  & \textbf{0.393} & 0.395 & \textbf{0.402} & \textbf{0.479}  \\
&   &  mr-quac\&quac & 0.388  & \textbf{0.401}  & 0.331 & 0.402  \\
        \cline{2-7}
 & unanswerable & quac & 0.843   & 0.852  & 0.805  & 0.844  \\
 &  (335)            & mr-quac & 0.527  & 0.550  & 0.440  & 0.540 \\
&  & mr-quac\&quac & 0.828 & 0.838 & 0.787  & 0.830  \\\hline
Merlinite-7B & answerable & quac & 0.367 & 0.382 & 0.282 & 0.368 \\
   & (665) & mr-quac & \textbf{0.394} & \textbf{0.393} & \textbf{0.431} & \textbf{0.509} \\
   &  & mr-quac\&quac & 0.372 & 0.385  & 0.300 & 0.378 \\
          \cline{2-7}
    & unanswerable & quac & 0.879 & 0.888 & 0.852 & 0.881 \\
    & (335) & mr-quac & 0.467 & 0.494 & 0.366 & 0.479 \\
   & & mr-quac\&quac & 0.867 & 0.876 & 0.838 & 0.869 \\\hline

\textbf{OR-QuAC}            \\\hline
LlaMA-13B-Chat & answerable & or-quac  & 0.145 & 0.149 & 0.133 & 0.153 \\
 & (4421)  &  dr-quac  & \textbf{0.153} & \textbf{0.154}  & \textbf{0.163} & \textbf{0.187} \\
&   &  dr-\&or-quac & 0.150  & 0.153   & 0.133 & 0.156  \\
        \cline{2-7}
 & unanswerable & or-quac & 0.799   & 0.799  & 0.799  & 0.799  \\
 &  (1150)  & dr-quac & 0.468  &  0.465  & 0.469  & 0.472 \\
&  & dr-\&or-quac & 0.787 & 0.787  & 0.787  & 0.787 \\\hline
Merlinite-7B & answerable & or-quac & 0.142  & 0.145 & 0.130  & 0.149 \\
   & (4421) & dr-quac & \textbf{0.199} & \textbf{0.197} & \textbf{0.233} & \textbf{0.265} \\
  &  & dr-\&or-quac & 0.146 & 0.148   & 0.137 & 0.154  \\
          \cline{2-7}
    & unanswerable & or-quac & 0.841  & 0.841 & 0.841 & 0.841  \\
    & (1150) & dr-quac & 0.215  & 0.215 & 0.216 & 0.217  \\
   & & dr-\&or-quac & 0.854 & 0.854  & 0.854 & 0.854 \\\hline

\textbf{MD2D}            \\\hline
LlaMA-13B-Chat & answerable & md2d  & 0.406 &	0.389 &	0.376 &	0.407 \\
 & (6178)  &               mr-md2d  & \textbf{0.429} &	\textbf{0.407} & \textbf{0.412} &	\textbf{0.493} \\
&   &                    mr-\&md2d  &  0.422 &	0.404 &	0.392 &	0.424   \\
        \cline{2-7}
 & unanswerable & md2d &  0.766 &	0.753 &	0.779 &	0.755  \\
 &  (4026)   & mr-md2d &  0.461 & 0.441 &	0.580 &	0.611 \\
&  &         mr-\&md2d & 0.758 & 0.745 &	0.768 &	0.742  \\\hline
Merlinite-7B & answerable & md2d  & 0.409 &	0.392 &	0.394 &	0.430  \\
 & (6178)  &               mr-md2d  & \textbf{0.439} & \textbf{0.421} & \textbf{0.415} & 0.450\\
&   &                    mr-\&md2d  & 0.415 &	0.419 &	0.410 &	\textbf{0.513}  \\
        \cline{2-7}
 & unanswerable & md2d &  0.769 &	0.756 &	0.787 &	0.765  \\
 &  (4026)   & mr-md2d &  0.410 &	0.403 &	0.546 &	0.585  \\
&  &         mr-\&md2d & 0.738  &	0.725 &	0.754 &	0.733  \\\hline

\textbf{CoQA}            \\\hline
LlaMA-13B-Chat & answerable & coqa  & 0.378 &	0.379 &	0.088 &	0.320	 \\
 & (7918)  &               mr-coqa  & \textbf{0.430} &	\textbf{0.430} &	\textbf{0.226} &	\textbf{0.428}   \\
&   &                    mr-\&coqa  & 0.400 &	0.382 &	0.193 &	0.363  \\
        \cline{2-7}
 & unanswerable & coqa   & 0.139 &	0.139 &	0.159 &	0.139	  \\
 &  (65)   & mr-coqa     & 0.015 &	0.015 &	0.109 &	0.015  \\
&  &         mr-\&coqa   & 0.139 &	0.139 &	0.152 &	0.139   \\\hline
Merlinite-7B & answerable & coqa  &  0.381 &	0.384 &	0.092 &	0.323  \\
 & (7918)  &             mr-coqa  &  \textbf{0.445} &	\textbf{0.441} &	\textbf{0.311} &	\textbf{0.499}  \\
&   &                  mr-\&coqa  &  0.412 &	0.384 &	0.202 &	0.383	\\
        \cline{2-7}
 & unanswerable & coqa &  0.108 &	0.108 &	0.113 &	0.108  \\
 &  (65)   & mr-coqa &  0.015 &	0.015 &	0.099 &	0.015 \\
&  &         mr-\&coqa &  0.092	 & 0.092 &	0.102 &	0.092  \\\hline



\end{tabular}
\caption{Benchmark testset performance of according to answerable vs. unanswerable query types. Comparison is between models instruction-tuned on human annotated training data only vs. synthetic data only. For answerable queries, models fine-tuned only on synthetic data out-perform those fine-tuned on human annotated data or combination of the two.}
\label{tab:answerable-vs-unanswerable-results}
\end{table*}
\end{comment}

==> rag-algorithm.tex <==
\begin{algorithm}[h]
\small
\caption{Multi-document Grounded Dialog Generation}
\label{alg:rag-dialog-algorithm}
\textbf{Input}: Initial user query $q_{1}$ from Algorithm~\ref{alg:mrc-dialog-algorithm} \\
\textbf{Output}: $dialog_{n}$ \& $passages_{m}$ \\
%\indent $n$=number of user and agent turns \\
%\indent $m$=number of unique retrieved passages \\
%\vspace{1mm}
\begin{algorithmic}[1]
\STATE $history \leftarrow \phi$ ; $passage_{m} \leftarrow \phi$

\FOR{ i = 1}
\STATE $passage_{1,k} \leftarrow retriever(q_{1})$ \\
\STATE $passage_{m} \leftarrow passage_{1,k}$ \\
\STATE $r_{1}\leftarrow LLM(q_{1},passage_{m})$ \\
\STATE $history_{1} \leftarrow q_{1}~\cup~r_{1}$ \\
\ENDFOR

\FOR {$i$ in $2~...~n$}
\STATE $q_{i}\leftarrow LLM(history_{i-1}, passage_{m})$
\STATE $passage_{i,k} \leftarrow retriever(q_{i}, history_{i-1})$
  \FOR {$j$ in $1~...~k$}
    \IF {$passage_{i,j} \notin passage_{m}$}
      \STATE $passage_{m} \leftarrow passage_{m} ~\cup~passage_{i,j}$
    \ENDIF
  \ENDFOR
\STATE $r_{i} = LLM(q_{i}, history_{i-1}, passage_{m})$
\STATE $history_{i} \leftarrow 
 history_{i-1} \cup q_{i} \cup r_{i}$

\ENDFOR
\STATE $dialog_{n} \leftarrow history_{n}$
\STATE return $dialog_{n}~\&~passage_{m}$
\end{algorithmic}
\end{algorithm}



==> sdg_humaneval_table.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{ccccccc}\\\hline
\textbf{Dialog Length}  & \textbf{\#Dialog} & \textbf{\%correct} & \textbf{\%answerable} & \textbf{\%plausible} & \textbf{\%diverse} & \textbf{\%coherent} \\\hline
1 turn & 100 & 75.6 & 85.2 & 93.4 & na &  na\\
2 turns & 60  & 73.1 & 87.4 & 98.9 & 98.9 & 100.0 \\
3 turns & 60  & 62.1 & 78.1 & 96.2 &92.9 & 95.0 \\
4 turns & 58  & 76.3 & 88.4 & 98.0 & 98.0 & 95.0 \\
5 turns & 16  & 88.8 & 93.8 & 99.4 & 90.6 & 93.8 \\\hline
Overall  & 294 & 73.1 & 85.2 & 96.7 & 95.6 & 96.7 \\\hline
\end{tabular}
\caption{Human evaluation of synthetic data quality according to dialog length. Dialog length 10 indicates 10 user queries plus 10 agent responses. \%diverse and \%coherent are applicable only to dialogs with 2 turns or more. Each sample has been evaluated by 2 or more annotators.}
\label{tab:sdg-human-evaluation-results}
\end{table*}
% chie-eva: 90% (45/50) 
% chie-heedong:74% (37/50) + 57% (34/60)
% eva-heedong:74% (37/50)
% roxana-chie: 77% (46/60)
% roxana-eva: 72% (43/60)
% heedong-roxana: 40% (24/60) + 43% (26/60)
\begin{comment}
\begin{table}
\centering
\begin{tabular}{ccccccc}\\\hline
turn depth  & \# turns & \%correct & \%answerable  \\\hline
1 & 100 & 76.8 & 87.5 \\
2  & 120  & 68.2 & 83.7 \\
3  & 180  & 66.4 & 79.3  \\
4  & 232  & 77.9 & 87.8 \\
5  & 80  & 84.4 & 93.8  \\\hline
Overall  & 712 & 73.1 & 85.2  \\\hline
\end{tabular}
\caption{Synthetic data quality human evaluation scores according to dialog turn depth with regard to the response correctness and query answerability. Correlation between the two is evident. Out of the 1270 annotations with answerable queries, 1062 (83.6\%) had correct answers, as opposed to the overall 73.1 \%correct.}
\label{tab:correlation-between-answerability-correctness}
\end{table}

\begin{table}
\centering
\begin{tabular}{llll}\\\hline
           &  \textbf{E} & \textbf{H} & \textbf{R} \\\hline
\textbf{C} & 90 (45/50) & 65 (71/110) & 77 (46/60) \\
\textbf{E} &         & 74 (37/50) & 72 (43/60) \\
\textbf{H} &         &       & 42 (50/120) \\\hline
\end{tabular}
\caption{Inter-annotator agreement (IAA) w.r.t the response correctness across 4 annotators, C, E, H and R. Included in parentheses are raw numbers. Agreement rate ranges from the lowest 42\% to the highest 90\%.}
\label{tab:IAA}
\end{table}

\end{comment}
